Can Large Language Models do Analytical Reasoning?

This paper explores the cutting-edge Large Language Model with analytical reasoning on sports. Our analytical reasoning embodies the tasks of letting large language models count how many points each team scores in a quarter in the NBA and NFL games. Our major discoveries are in two folds. Firstly, we find among all the models we employed, GPT-4 stands out in effectiveness, followed by Claude-2.1, with GPT-3.5, Gemini-Pro, and Llama-2-70b lagging behind. Specifically, we compare three different prompting techniques and a divide-and-conquer approach, we find that the latter was the most effective. Our divide-and-conquer approach breaks down play-by-play data into smaller, more manageable segments, solves each piece individually, and then aggregates them together. Besides the divide-and-conquer approach, we also explore the Chain of Thought (CoT) strategy, which markedly improves outcomes for certain models, notably GPT-4 and Claude-2.1, with their accuracy rates increasing significantly. However, the CoT strategy has negligible or even detrimental effects on the performance of other models like GPT-3.5 and Gemini-Pro. Secondly, to our surprise, we observe that most models, including GPT-4, struggle to accurately count the total scores for NBA quarters despite showing strong performance in counting NFL quarter scores. This leads us to further investigate the factors that impact the complexity of analytical reasoning tasks with extensive experiments, through which we conclude that task complexity depends on the length of context, the information density, and the presence of related information. Our research provides valuable insights into the complexity of analytical reasoning tasks and potential directions for developing future large language models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/7_Others.tex <==
\section*{Author Contributions}
If you'd like to, you may include a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\section*{Acknowledgments}
Use unnumbered third-level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> tables/main_results_nba.tex <==
\begin{table*}[htbp]
    \centering
    \small
    \begin{tabular}{lrrrrrrrrrr}
    \toprule[1pt]
    \multicolumn{1}{c}{Models} & \multicolumn{2}{c}{GPT-3.5} & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c}{Claude-2.1} & \multicolumn{2}{c}{Gemini-Pro} & \multicolumn{2}{c}{Llama-2-70b} \\
    \cmidrule{2-11}
    \multicolumn{1}{c}{Methods} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} \\
    \midrule
    NL Inst. & \textbf{4.45} & \textbf{14.00} & 4.08 & 18.18 & 3.02 & 16.62 & 2.49 & 42.87 & 3.21 & \textbf{22.25}\\
    \quad +\textsc{JSON} & 3.59 & 15.99 & 11.26 & 7.84 & 4.33 & 17.41 & \textbf{2.83} & 41.49 & 4.34 & 19.34\\
    \quad +\textsc{COT} & 2.37 & 19.84 & \textbf{40.47} & \textbf{2.74} & \textbf{16.96} & \textbf{13.12} & 2.60 & \textbf{41.13} & \textbf{4.84} & 21.11 \\
    \midrule
    DnC(n=1) & 1.00 & 15.26 & 20.54 & 30.84 & \textbf{32.67} & 11.74 & 3.71 & \textcolor{red}{$>$100} & 0.00 & \textcolor{red}{$>$100} \\
    DnC(n=3) & \textbf{16.58} & \textbf{4.39} & \textbf{60.14} & \textbf{1.70} & 29.46 & \textbf{5.48} & \textbf{26.23} & 14.12 & \textbf{6.44} & \textcolor{red}{$>$100} \\
    DnC(n=10) & 0.24 & 19.87 & 38.37 & 2.24 & 12.87 & 7.65 & 4.46 & \textbf{13.69} & 4.14 & \textbf{57.80}\\
    DnC(n=30) & 0.70 & 28.20 & 18.31 & 4.86 & 2.23 & 14.56 & 1.48 & 35.54 & 0.99 & \textcolor{red}{$>$100} \\
    \bottomrule[1pt]
    \end{tabular}
    \caption{\small Total Score Results on NBA quarters. The best performance results in both the prompting and planning-based methods are \textbf{bolded}. (\textcolor{red}{RED}) We found that the Llama-2-70b model usually hallucinates the total scores when doing step-by-step updating.}
    \label{tab: NBA results}
    \vspace{-0.2in}
\end{table*}


==> tables/main_results_nfl.tex <==
\begin{table*}[htbp]
    \centering
    \small
    \begin{tabular}{lrrrrrrrrrr}
    \toprule[1pt]
    \multicolumn{1}{c}{Models} & \multicolumn{2}{c}{GPT-3.5} & \multicolumn{2}{c}{GPT-4} & \multicolumn{2}{c}{Claude-2.1} & \multicolumn{2}{c}{Gemini-Pro} & \multicolumn{2}{c}{Llama-2-70b} \\
    \cmidrule{2-11}
    \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} & \multicolumn{1}{c}{\texttt{$\uparrow$ACC}} & \multicolumn{1}{c}{\texttt{$\downarrow$MAPE}} \\
    \midrule
    NL Inst. & 45.38 & 29.27 & 55.38 & 24.01 & 45.69 & 30.84 & \textbf{35.32} & \textbf{35.71} & 33.54 & 43.44\\
    \quad +\textsc{JSON} & \textbf{50.41} & 29.50 & \textbf{57.38} & \textbf{23.92} & 53.02 & 27.01 & 35.13 & 42.00 & \textbf{35.87} & \textbf{38.80} \\
    \quad +\textsc{COT} & 48.00 & \textbf{27.56} & 55.91 & 25.39 & \textbf{56.68} & \textbf{23.59} & 33.02 & 40.06 & 31.53 & 46.07 \\
    \midrule
    Plan(n=1) & 39.50 & \textcolor{red}{$>$100} & 95.76 & 2.31 & \textbf{85.39} & \textbf{7.84} & \textbf{60.50} & \textbf{17.24} & 5.29 & \textcolor{red}{$>$100} \\
    Plan(n=3) & \textbf{81.25} & 14.39 & 98.25 & 1.08 & 71.53 & 18.23 & 51.00 & 22.40 & 9.82 & \textcolor{red}{$>$100} \\
    Plan(n=10) & \textbf{81.25} & \textbf{9.49} & \textbf{98.77} & \textbf{0.66} & 81.61 & 10.58 & 49.23 & 17.44 & 36.75 & \textcolor{red}{$>$100}\\
    Plan(n=30) & 79.50 & 15.23 & 97.00 & 1.13 & 76.50 & 10.64 & 50.46 & 21.81 & \textbf{52.25} & \textbf{37.63} \\
    \bottomrule[1pt]
    \end{tabular}
    \caption{\small Total Score Results on NFL quarters. The best performance results in both the prompting and planning-based methods are \textbf{bolded}. We found that Llama-2-70b and GPT-3.5 usually hallucinates a final scores during the reasoning on single step. High MAPE, as labeled in (\textcolor{red}{RED}), indicates high possibility of hallucinations.}
    \label{tab: NFL results}
\end{table*}


==> tables/prompt_example.tex <==
\begin{table*}[htbp]
    \centering
    \small
    \begin{tabular}{|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|}
    \hline
    \multicolumn{6}{l}{\textbf{System Message}} \\
    \hline
    %\multicolumn{3}{p{7.5cm}}{\textbf{NBA:}} & \multicolumn{3}{p{7.5cm}}{\textbf{NFL:}} \\
    \multicolumn{6}{p{15cm}}{You are a helpful assistant tasked with analyzing sports games.
    You have been given a play-by-play breakdown of \textbf{[\texttt{an NBA basketball} / \texttt{an NFL football}]} game between two teams.
    \newline
    \newline
    The "Time" column shows the exact time on the game clock when each play took place. The game clock counts down, so this column displays times in a descending order.
    \newline
    \newline
    The "Play" column describes the action that happened at the respective times. It provides details of specific plays, movements, and outcomes on the court.
    \newline
    \newline
    Team players are listed in two rows, each row representing one of the two \textbf{[\texttt{basketball} / \texttt{football}]} teams involved in the game.}
    %& \multicolumn{3}{p{7.5cm}}{You are a helpful assistant tasked with analyzing sports games.
    %You have been given a play-by-play breakdown of a NFL football game between two teams.
    %\newline
    %\newline
    %The "Time" column shows the exact time on the game clock when each play took place. The game clock counts %down, so this column displays times in a descending order.
    %\newline
    %\newline
    %The "Play" column describes the action that happened at the respective times. It provides details of %specific plays, movements, and outcomes on the court.
    %\newline
    %\newline
    %Team players are listed in two rows, each row representing one of the two NFL teams involved in the game.}
    \\
    \hline
    \multicolumn{6}{l}{\textbf{User Message}} \\
    \hline
    \multicolumn{2}{p{5cm}|}{\textbf{Natural Instruction}} &
    \multicolumn{2}{p{5cm}|}{\textbf{Natural Language Instruction \newline + \textsc{JSON} Format}} &
    \multicolumn{2}{p{5cm}}{\textbf{Natural Language Instruction \newline + COT}} \\
    \hline
    \multicolumn{2}{p{5cm}|}{How many points did each team score in the given game input? Return 0 if no team scored. Don't present the calculation process.} &
    \multicolumn{2}{p{5cm}|}{How many points did each team score in the given game input? Only response in JSON format as below.} &
    \multicolumn{2}{p{5cm}}{How many points did each team score in the given game input? Let's think step by step.} \\
    \hline
    \multicolumn{6}{l}{\textbf{Context}} \\
    \hline
    \multicolumn{6}{l}{Initial Scores:} \\
    \multicolumn{6}{p{15cm}}{\{"New York Knicks": 0, "Denver Nuggets": 0\}\newline}\\
    %\hline
    %\multicolumn{6}{l}{\textbf{Affiliation Data}} \\
    %\hline
    \multicolumn{6}{p{15cm}}{Team-Player Table:
    \newline
    New York Knicks: Kenyon Martin, Carmelo Anthony, Andrea Bargnani, Raymond Felton, Iman Shumpert, Metta World Peace, Tim Hardaway JR., Amare Stoudemire, Beno Udrih, Pablo Prigioni, J.R. Smith
    \newline
    Denver Nuggets: Wilson Chandler, Kenneth Faried, J.J. Hickson, Randy Foye, T.Y. Lawson, Darrell Arthur, Timofey Mozgov, Andre Miller, Nate Robinson, Jordan Hamilton, Evan Fournier\newline} \\
    \multicolumn{6}{l}{Game Input:} \\
    \multicolumn{1}{p{2.5cm}}{
    Time\newline
    12:00\newline
    11:40\newline
    11:22}
    & \multicolumn{5}{p{12.5cm}}{
    Play\newline
    Carmelo Anthony vs. J.J. Hickson (Kenneth Faried gains possession)\newline
    Randy Foye makes driving layup\newline
    Carmelo Anthony misses 18-foot jumper}\\
    \hline
    \end{tabular}
    \caption{An example of three prompting-based methods.}
    \label{tab: prompt_example}
\end{table*}
